Dynamic Spectrum Sharing in the Age of Millimeter Wave Spectrum Access

Next-generation wireless networks are facing spectrum shortage challenges, mainly due to, among other factors, the projected massive numbers of IoT connections and the emerging bandwidth-hungry applications that such networks ought to serve. Spectrum is scarce and expensive, and therefore, it is of crucial importance to devise dynamic and flexible spectrum access policies and techniques that yield optimal usage of such a precious resource. A new trend recently being adopted as a key solution to this spectrum scarcity challenge is to exploit higher frequency bands, namely mmWave bands, that were considered impractical few years ago, but are now becoming feasible due to recent advances in electronics. Though, fortunately, spectrum regulatory bodies have responded by allowing the use of new bands in the mmWave frequencies, much work still needs to be done to benefit from such new spectra. In this paper, we discuss some key spectrum management challenges that pertain to dynamic spectrum access at the mmWave frequencies, which need to be overcome in order to promote dynamic spectrum sharing at these mmWave bands. We also propose new techniques that enable efficient dynamic spectrum sharing at the mmWave bands by addressing some of the discussed challenges, and highlight open research challenges that still need to be addressed to fully unleash the potential of dynamic spectrum sharing at mmWave bands.

==> challenges.tex <==
This project focuses on addressing the following 5G spectrum efficiency challenges:
\begin{itemize}

\item {\bf Challenge 1- Spectrum usage heterogeneity:} Multiple different types of 5G devices, running various applications with different QoS requirements and traffic demands, will be connected to and supported by the 5G network infrastructure. This diversity will result in heterogeneous access to the 5G's wideband spectrum, where different bands will experience different occupancy and usage behaviors with variability across time, frequency, and space.

\item {\bf Challenge 2- Ultra-wideband (sub-6GHz \& mmWave) spectrum access:} The spectrum bands opened up for 5G span a wide range of frequencies, ranging from low-frequency ($\leq$ 1 GHz) to high-frequency (mmWave/above-24 GHz) bands. The wideband nature of this spectrum renders existing spectrum availability recovery approaches---mainly designed for narrowband access---inefficient. For instance, transmissions at mmWave frequencies are subject to high signal path losses, potentially leading to high false positives of spectrum occupancy information.
    %, where devices may perceive that a given band is available due to the lack of primary signals, even though the band may not be available in reality.

\item {\bf Challenge 3- Limited hardware capability:}
   Wideband spectrum usage varies over time and from one frequency band to another, making existing spectrum availability recovery techniques, which leverage spectrum occupancy variability to provide efficient recovery, suffer from current hardware limitations. This leads to inaccurate and unreliable recovery of spectrum availability information.

\item {\bf Challenge 4- Traffic jams at the network edges:} The high user density, the high bandwidth demand, and the massive device connectivity requirements of 5G will create severe traffic congestion bottlenecks at the backhaul links in both the downlink and uplink directions.

\end{itemize}


